Gyrokinetic simulations of plasma turbulence in a Z-pinch using a moment based approach and advanced collision operators

The first nonlinear gyrokinetic simulations obtained using a moment approach based on the Hermite-Laguerre decomposition of the distribution function are presented, implementing advanced models for the collision operator. Turbulence in a \modif{two-dimensional} Z-pinch is considered within a flux tube configuration. In the collisionless regime, our gyromoment approach shows very good agreement with nonlinear simulations carried out with the continuum gyrokinetic code GENE, even with fewer gyromoments than required for the convergence of the linear growth rate. By using advanced linear collision operators, the role of collisions in setting the level of turbulent transport is then analyzed. The choice of collision operator model is shown to have a crucial impact when turbulence is quenched by the presence of zonal flows. The convergence properties of the gyromoment approach improve when collisions are included.

==> A1_hermite_laguerre_basis.tex <==
\section{Hermite Laguerre basis and kernel function}
\label{se:hermite_laguerre}
\subsection{Hermite Polynomials}
The normalized Hermite polynomials can be defined by 
\begin{equation}
    H_p[x] = (-1)^p e^{x^2} \frac{d^p}{dx^p}e^{-x^2} = \sqrt{2^p p!} \hat{H}_p[x]
\end{equation}
where $\hhat_p$ is the normalized Hermite polynomial. 
These are orthogonal w.r.t. an inner product weighted by an exponential $e^{-x^2}$, i.e.
\begin{equation}
    \langle \hhat_p, \hhat_{p'}\rangle_H = \int \hhat_p[x] \hhat_{p'}[x] e^{-x^2}dx = \delta_{pp'}.
    \label{eq:hermite_orthogonality}
\end{equation}
One can notice the useful argument product recurrence relation 
\begin{equation}
    x\hhat_p = \sqrt{\frac{p+1}{2}} \hhat_{p+1} + \sqrt{\frac{p}{2}}\hhat_{p-1}.
    \label{eq:hermite_arg_prod}
\end{equation}
The derivative of Hermite polynomials follows the recursive rule 
\begin{equation}
    H'_p = 2p H_{p-1} \quad\textrm{or}\quad \hat H'_p = \sqrt{2p}\hat H_{p-1}
\end{equation}
for normalized polynomials. We can extend this rule to the $d$-th derivative as
\begin{equation}
    \hat H^{(d)}_p = 2^{d/2}\sqrt{\frac{p!}{(p-d)!}}\hat H_{p-d}.
    \label{eq:hermite_derivative}
\end{equation}
We usually omit the hat of $\hat H_p$ and write $H_p$ as it contains the normalization factor.
\subsection{Laguerre Polynomials}
The Laguerre polynomials are defined as
\begin{equation}
    L_j[x] = \frac{e^x}{j!}\frac{d^j}{dx^j}(e^{-x}x^j) = \sum_{n=0}^j\frac{j!}{(j-n)!n!}\frac{(-1)^n}{n!}x^n
\end{equation}
and are orthonormal to a $e^{-x}$ weighted inner product, i.e.
\begin{equation}
    \langle L_j,L_{j'}\rangle_L = \int L_j[x] L_{j'}[x] e^{-x}dx = \delta_{jj'}.
    \label{eq:laguerre_orthogonality}
\end{equation} 
Laguerre polynomials fulfill the following argument product recurrence relation
\begin{equation}
    x L_j = (2j+1)L_j - j L_{j-1} - (j+1) L_{j+1}.
    \label{eq:laguerre_arg_prod}
\end{equation}
For perpendicular velocity nonlinearities, it is useful to note that the product of two Laguerre polynomials can be reduced as
\begin{equation}
 L_n^m L_k = \sum_{s=0}^{n+k}\overline{d}_{nks}^m L_s
 \label{eq:laguerre_product_id}
\end{equation}
with the coefficients
$$
\overline{d}^{|m|}_{nkf} = \sum_{n_1 = 0}^n \sum_{k_1 =0}^k   \sum_{f_1=0}^f L_{kk_1}  L_{nn_1}^{|m|}  L_{f f_1} (n_1 + k_1 + f_1)!
$$
where  $L^{c}_{ab}$ is the $b$-th degree polynomial coefficient of $L^{c}_a$. The associated Laguerre polynomial of degree $a$ can be written explicitly as
\begin{equation}
 L^{m}_j(x) = \sum_{l=0}^j L^m_{jl} x^l\quad\textrm{where}\quad L_{jl}^m= \frac{(j+m)!}{(j-l)!(l+m)!}\frac{(-1)^l}{l!}.
 \label{eq:laguerre_exp_form}
\end{equation}
One can now write the $d_{njs}$ coefficients as
\begin{equation}
    d_{njs} = \sum_{n_1}^n\sum_{j_1}^j\sum_{s_1}^s (-1)^{n_1+j_1+s_1} \frac{n!j!s!}{n_1!j_1!s_1!}\frac{(n_1+j_1+s_1)!}{(n-n_1)!(j-j_1)!(s-s_1)!}.
\end{equation}
Let us also recall the Laguerre derivative rule
\begin{equation}
    L_j' = L_{j-1}' - L_{j-1} = -\sum_{l=0}^{j-1}L_{l}.
\end{equation}
which we can then extend it for the nth derivatives as
\begin{align}
    L_j^{(d)}&= (-1)^d\sum_{l=0}^{j-d}\binom{j-(l+1)}{d-1}L_l.\label{eq:laguerre_derivative}
\end{align}
(\textit{Identity \eqref{eq:laguerre_derivative} is not verified but I think it's correct, no ref has been found but possible to demonstrate it by induction.})

\subsection{Kernel functions}
In the gyromoment model, the Bessel's function of the first kind $J_0$ is projected to the Laguerre basis using the relation \begin{equation}
    J_0[\kperp\vperp] = \sum_{n=0}^{\infty}\kernel_n[\kperp\rho_{tha}/2] L_n[\sperpa^2]
    \label{eq:bessel_laguerre_id}
\end{equation} 
which is exact when defining the kernel functions as
\begin{equation}
    \kernel_n(x) = \frac{1}{n!}\roundparenthesis{\frac{x}{2}}^{2n}e^{-(x/2)^2} \underset{y=(x/2)^2}{=}  \frac{y^{n}}{n!}e^{-y}
    \label{eq:kernel_def}
\end{equation}
or recursively for more efficient computation
\begin{equation}
    \kernel_0(y) = e^{-y},\quad \kernel_{j+1}(y) = \frac{y}{j+1}\kernel_j(y).
    \label{eq:kernel_def_rec}
\end{equation}
In our framework, the non dimensional argument of the kernel function is expressed as
\begin{equation}
    y=\roundparenthesis{\frac{b_a}{2}}^2 =\frac{1}{4}(\sigma_a\sqrt{2\tau_a}\kperp)^2 = \frac{\sigma_a^2\tau_a}{2}\kperp^2.
\end{equation}
Since equation \eqref{eq:bessel_laguerre_id} is exact only for an infinite sum, the finite number of Laguerre polynomials $J_{max}$ used in \texttt{HeLaZ} will induce a truncation error. It is worth noting that those errors are negligible for high polynomial degree since $\kernel_n\sim 1/n!$ for $n \gg 1$. However, investigations should be made on alternative expression of $\kernel_n$ that would lead to better behavior of the finite sum at $J_{max} < 10$.


\subsection{Hermite-Laguerre moments definition}
Let us define the projection on Hermite Laguerre polynomial basis as the norm
\begin{equation}
    ||\chi||_a^{pj} =\int d^3v\,\chi\,\hhat_p[\spara] L_j[x_a].
    \label{eq:apj_norm}
\end{equation}
In our framework, the kinetic distribution function is gyro-averaged and close to a Maxwellian, i.e. $f_a \rightarrow  \langle f_a \rangle_{\theta} \sim \FaM + \delta f_a$. Thus the perturbed gyro-moment of degree $p,j$ is given by
\begin{equation}
     N_a^{pj} = ||g_a||_a^{pj} =\int d^3v\,g_a \,\hhat_p[\spara] L_j[x_a]
    \label{eq:gyromom_def}   
\end{equation}
in Fourier modes.

\subsection{Fluid moments equivalences}
In order to obtain the fluid moments, one has to take into account that the gyro moments are defined for gyro-centers and related, at first order, to the Bessel function $J_0$. For example, particle density fluctuation is obtained using \eqref{eq:bessel_laguerre_id} which in Fourier space yields
\begin{equation}
    \delta n_a(\bm x,t) =  \int d^3v \,J_0 h_a(\bm k,t) H_0 L_0 = \sum_{l=0}^\infty \kernel_l n_a^{0,l}
    \label{eq:fluid_density}
\end{equation}
with $h_a := g_a +\tau_a/q_a J_0 \phi$ the nonadiabatic part of the distribution function and $n_a^{pj}:= N_a^{pj} + \tau_a/q_a\kernel_j\phi\delta_p^0$ the non adiabatic gyromoments.
The same recipe for higher fluid moments yields
\begin{equation}
    \delta u_{\parallel a} = \sum_{l=0}^\infty \kernel_l n_a^{1l},\qquad \delta u_{\perp a} = b_a\sum_{n=0}^\infty\frac{1}{2} [\kernel_n-\kernel_{n-1}] n_a^{0n}
    \label{eq:fluid_velocity}
\end{equation}
for parallel and perpendicular fluid velocity and
\begin{equation}
    \delta T_{\parallel a} = \sum_{l=0}^\infty \kernel_l [\sqrt 2 n_a^{2,l}+n_a^{0,l}],\qquad  \delta T_{\perp a} = \sum_{l=0}^\infty [(2l+1)\kernel_l - (l+1) \kernel_{l+1} - n\kernel_{l-1}]n_a^{0,l}.
    \label{eq:fluid_temperature}
\end{equation}
for parallel and perpendicular temperature, respectively.

==> GS2_model.tex <==
\section{GS2 model}
GS2 code solves the non-linear gyrokinetic equation for the non-adiabatic part of the perturbed distribution function $\dfa$ using the Vlasov equation
\begin{equation}
    \ddt \dfa + [\chi,\dfa] + \vpar\bvec\cdot\grad\dfa + i\omega_d \dfa = i\omega^*\chi - e\partial_E F_0 \ddt \chi
    \label{gs2vlasov}
\end{equation}
with the magnetic resonance frequency
\begin{equation}
    \omega_d = \bm{k}_\perp\cdot\roundparenthesis{\bm{B}\times\frac{m\vpar^2\bm\kappa + \mu \grad B}{B\Omega}} = \bm{k}_\perp \cdot \roundparenthesis{\bm{U}_{\kappa a}+\bm{U}_{\grad a}}.
\end{equation}
Sided with the electromagnetic fields contained in
\begin{equation}
    \chi = J_0 \roundparenthesis{\dphi - \frac{\vpar}{c}A_\parallel} + \frac{J_1}{\kperp \rho}\frac{m\vperp^2}{e}\frac{B_\parallel}{B}.
\end{equation}
which follow the Maxwell equations expressed here as GK Poisson-Ampere equations
\begin{align}
    \nabla^2_\perp\dphi &= 4\pi\sum_a e\int d\bm v \squareparenthesis{e\dphi\partial_E F_0 + J_0 \dfa}\\
    %
    \nabla^2_\perp A_\parallel &= -\frac{4\pi}{c}\sum_a \int d\bm v e\vpar J_0 \dphi\\
    %
     \label{gs2magn}\frac{B_\parallel}{B} &= -\frac{4\pi}{B^2}\sum_a \int d\bm v m_a \vperp^2 \frac{J_1}{\kperp\rho}\dfa
\end{align}
equations \eqref{gs2vlasov} to \eqref{gs2magn} are self-consistent.\\ The Poisson bracket term of the Vlasov equation \eqref{gs2vlasov} contains the non-linear part of such system as
\begin{equation}
    [\chi,\dfa] = \grad_v\dfa\cdot\grad_x\chi - \grad_v\chi\cdot\grad_x\dfa
\end{equation}

==> backup.tex <==
% \begin{align}
%     &\ddt N_a^{pj}+ \frac{\tau_a}{q_a} i k_y \squareparenthesis{\sqrt{(p+1)(p+2)} n_a^{p+2,j} + (2p+1)n_a^{p,j} + \sqrt{p(p-1)}n_a^{p-2,j}}\nonumber\\
%     %
%     &+ \frac{\tau_a}{q_a} i k_y \squareparenthesis{(2j+1)n_a^{pj} - (j+1)n_a^{p,j+1}-jn_a^{p,j-1}}\nonumber\\
%     %
%     &-\kappa_N ik_y\phi\squareparenthesis{\roundparenthesis{1-\frac{3}{2}\eta}\kernel_j\delta_{p}^0 + \eta\kernel_j\roundparenthesis{\frac{1}{2}\delta_p^0 + \frac{1}{\sqrt{2}}\delta_p^2} + \eta([2j+1]\kernel_j-[j+1]\kernel_{j+1}-j\kernel_{j-1})\delta_p^0} \nonumber\\
%     &=\sum_{ab}C_{ab}^{pj}+\squareparenthesis{\sum_{n=0}^{\infty}\roundparenthesis{ik_x\kernel_n\phi}*\roundparenthesis{ik_y\sum_{s=0}^{n+j}d_{njs}N_a^{ps}} - \roundparenthesis{ik_y\kernel_n\phi}*\roundparenthesis{ik_x\sum_{s=0}^{n+j}d_{njs}N_a^{ps}}}
%     \label{eq:moment_gyboeq_nondim_nonadiab}.
% \end{align}
% We use, in equation \eqref{eq:moment_gyboeq_nondim_nonadiab}, the magnetic gradient length $L_{\textrm{ref}}=L_B$ as reference length and the sound Larmor radius for the typical fluctuation scale, i.e. $k_{x,y,\textrm{ref}}=1/\rho_s= \Omega_i/c_s$ where $c_s=\sqrt{T_e/m_i}$ is the sound speed and $\Omega_i=\sqrt{eB/m_i}$ the ion cyclotron frequency. 
% We also introduce the dimensionless temperature and mass ratios, i.e. $\tau_a=T_a/T_i$ and $\sigma_a=\sqrt{m_a/m_i}$, respectively.

==> dimensions.tex <==
\topmargin=-0.45in      %
%\evensidemargin=0in     %
\oddsidemargin=-0.1in      %
\textwidth=6.8in        %
\textheight=9.2in       %
%\headsep=0.25in         %
\headheight=30.9pt

==> nonlin_term.tex <==
\subsection{Moments equation right-hand-side : nonlinear term}
In the moments formulation \eqref{eq:moment_gyboeq_nondim}, we ended up with a nonlinear term that has to be treated carefully, i.e.
\begin{align}
    S_a^{pj} :&= ||\mathcal{F}[\grad \dphi \times \grad \dga ]||_a^{pj} \nonumber\\
    &= \epsilon^{-1}\int\sum_{n=0}^{\infty} \bvec\cdot\roundparenthesis{\phi[\bm k']\kernel_n[b']\bm k'\times (\bm k - \bm k')\sum_{s=0}^{n+j}d_{njs}N_a^{ps}[\bm k -\bm k']}d\bm k'
\end{align}
The high order $\epsilon^{-1}$ factor in front can be removed by normalizing our perturbation fields by $\epsilon$ so that $\phi \times N_a^{pj}\sim \epsilon^2$ and
resulting into a $\epsilon^1$ factor that simplifies with the linear terms ones.
Once this small normalization done, the nonlinear term can be written in a more explicit format as
\begin{align}
    &\int \sum_{n=0}^{\infty}(k_z'-k_r')\phitilde[\bm k']\kernel_n[b']((k_z-k_z')-(k_r-k_r'))\sum_{s=0}^{n+j}d_{njs}N_a^{ps}[\bm k -\bm k']d\bm k'\nonumber\\
    %
    &=\sum_{n=0}^{\infty}\int \underbrace{(k_z'-k_r')\phitilde[\bm k']\kernel_n[b']}_{\Phi_n[\bm k']}%
    \cdot\underbrace{(\Delta k_z'-\Delta k_r')\Sigma_{s=0}^{n+j}d_{njs}N_a^{ps}[\Delta\bm k']}_{\Gamma_{an}^{pj}[\bm k-\bm k']}d\bm k'\nonumber\\
    %
    &=\sum_{n=0}^{\infty} (\Phi_n *  \Gamma_{an}^{pj})[\bm k] %
    =\sum_{n=0}^{\infty}\mathcal{F}\roundparenthesis{\mathcal{F}^{-1}\squareparenthesis{\Phi_n} \cdot \mathcal{F}^{-1}\squareparenthesis{\Gamma_{an}^{pj}}}%
    =\mathcal{F}\roundparenthesis{\sum_{n=0}^{\infty}\mathcal{F}^{-1}\squareparenthesis{\Phi_n} \cdot \mathcal{F}^{-1}\squareparenthesis{\Gamma_{an}^{pj}}}
    \label{eq:2nd_term_convolution_th}
\end{align}
This notation points out the possibility to use Fourier transform instead of integrals thanks of the convolution theorem $\mathcal{F}[f * g] = \mathcal{F}[f] \cdot \mathcal{F}[g]$. It is worth noting that this formulation may be more computationally intense than the one in GS2 (\cite{Highcock2012}) where the derivatives were simply replaced by an inverse Fourier transform, i.e.
\begin{equation}
    \partial_z\phi \partial_r g = \mathcal{F}^{-1}[ik_z J_0 \phi] \cdot \mathcal{F}^{-1}[i k_r g].
\end{equation}
In our case, the Bessel function was projected on the Hermite-Laguerre basis which lead to the sum of kernel functions $\kernel_n$. 
\\
One can design a process that allows us to obtain the non-linear term $S_a^{pj}$ at a given wave vector $\bm k$ by using discrete fast Fourier transform (FFT), avoiding the convolution integral.
FFT consists in a transformation of a signal $\{f_j\}_{j=0}^{N-1}$ to a frequency spectrum $\{F_k\}_{k=0}^{N-1}$ as\footnote{The following development has inspired by \textit{How Important is Dealiasing for Turbulence Simulations?} from John C. Bowman, University of Alberta, September 30, 2014.}

\begin{equation}
    \mathrm{FFT}[f]_k = F_k = \frac{1}{N}\sum_{j=0}^{N-1}(\zeta_N)^{-kj}f_j
\end{equation}

and the inverse transform

\begin{equation}
    \mathrm{FFT}^{-1}[F]_j = f_j = \sum_{k=0}^{N-1}(\zeta_N)^{jk}F_k
\end{equation}
where the weights are defined $\zeta_N=e^{-2\pi i/N}$ and fulfill the relation
\begin{equation}
    \sum_{j=0}^{N-1}(\zeta_N)^{lj} = 
    \begin{cases}
    N& \text{if $l=sN$ for $s\in\mathbb{Z}$}\\
    0              & \text{otherwise}
    \end{cases}
    \label{eq:zeta_id}
\end{equation}
Thus in a one dimensional discrete case, our convolution term transformed in a real space product can be written as
\begin{align}
    (F*G)_k = \textrm{FFT}[f\cdot g]_k &=\sum_{j=0}^{N-1} f_{j} g_{j}(\zeta_N)^{-kj}\nonumber\\
    %
    &=\sum_{j=0}^{N-1} (\zeta_N)^{-kj} \sum_{l=0}^{N-1}(\zeta_N)^{jl}F_l \sum_{m=0}^{N-1}(\zeta_N)^{jm}G_m \nonumber\\
    & \sum_{l=0}^{N-1} F_l \sum_{m=0}^{N-1} G_m \sum_{j=0}^{N-1} (\zeta_N)^{(l+m-k)j}\nonumber\\
    %
    \rvert_\eqref{eq:zeta_id}&=N\sum_s\sum_{l=0}^{N-1}F_l G_{k-l+sN}
    \label{eq:aliasing}
\end{align}
Thus, it is important to notice that that in the discrete case, the convolution theorem lead to additional terms called aliases, corresponding to each $G_{k-l+sN}$ where $s\neq 0$. These terms will introduce unwanted errors in the computation of the linear term and must be removed by ensuring that $G_{k-l+sN} = 0$ whenever $s\neq 0$.\\
Practically, if $F_n$ and $G_n$ are nonzero only up to $n\leq M$, a non aliased convolution can be set up by extending our signal to $N \geq 2M -1$ since it will cancel each terms for $k-l+sN\geq M$.


In two dimensions the discrete convolution is derived in Appendix \ref{appendix:2D_aliasing} and is a simple extension from the 1D case leading to the anti-aliasing condition
\begin{equation*}
    G_{k_r - l_r + s_r N_r,k_z - l_z + s_z N_z} = 0 \quad \forall s_r,s_z\neq 0.
\end{equation*}
In conclusion, one can dealiase completely our 2D signal by zero padding the discretized expression of $\Phi_{an}$ and $\Pi_{an}^{pj}$ found in \eqref{eq:2nd_term_convolution_th}.
One can summarize the work done in this chapter by the following algorithm

\begin{algorithm}
\caption{Nonlinear term computation}
\label{alg:conv_FFT}
\begin{algorithmic}[ht]
    \STATE $\{S_a^{pj}\}_{k_r,k_z=0}^{M_r,M_z} \gets 0$
    \FORALL{$n=0,J_{max,a}-j$}
    \STATE $\{F_{k_r,k_z}\}_{k_r,k_z=0}^{N_r,N_z} \gets \{(k_z-k_r)\phitilde[\bm k]\kernel_n[b_a]\}_{k_r,k_z=0}^{N_r,N_z}$
    \STATE
    \STATE $\{G_{k_r,k_z}\}_{k_r,k_z=0}^{N_r,N_z} \gets \{(k_z-k_r)\sum_{s=0}^{n+j}d_{njs}N_a^{ps}[\bm k]\}_{k_r,k_z=0}^{N_r,N_z}$
    \STATE
    \STATE$\{F_{k_r,k_z}\}_{k_r,k_z=0}^{M_r,M_z} \gets $ zero padding$\roundparenthesis{\{F_{k_r,k_z}\}_{k_r,k_z=0}^{N_r,N_z},\, M = 2N -1}$
    \STATE
    \STATE$\{G_{k_r,k_z}\}_{k_r,k_z=0}^{M_r,M_z} \gets $ zero padding$\roundparenthesis{\{G_{k_r,k_z}\}_{k_r,k_z=0}^{N_r,N_z},\, M = 2N -1}$
    \STATE
    \STATE $\{f_{r,z}\}_{k_r,k_z=0}^{M_r,M_z} \gets \textrm{FFT}^{-1}\squareparenthesis{\{F_{k_r,k_z}\}_{k_r,k_z=0}^{M_r,M_z}}$
    \STATE
    \STATE $\{g_{r,z}\}_{k_r,k_z=0}^{M_r,M_z} \gets \textrm{FFT}^{-1}\squareparenthesis{\{G_{k_r,k_z}\}_{k_r,k_z=0}^{M_r,M_z}}$
    \STATE
    \STATE $\{S_a^{pj}\}_{k_r,k_z=0}^{M_r,M_z} \gets \{S_a^{pj}\}_{k_r,k_z=0}^{M_r,M_z} + \{f_{r,z}\cdot g_{r,z}\}_{k_r,k_z=0}^{M_r,M_z}$
    \ENDFOR
    \RETURN $\textrm{FFT}\squareparenthesis{\{S_a^{pj}\}_{k_r,k_z=0}^{N_r,N_z}}$
\end{algorithmic}
\end{algorithm}

This algorithm does not show however the truncation that is needed in order to compute the term $G$ since the $N_a^{ps}$ are defined up to $s = J_{max,a}$. Practically, it is achieved by setting the upper bound of the sum over $s$ to $min(J_{max,a},n+j)$, i.e.
$$
G = (k_z-k_r)\sum_{s=0}^{n+j}d_{njs}N_a^{ps}[\bm k] \approx (k_z-k_r)\sum_{s=0}^{min(n+j,J_{max,a})}d_{njs}N_a^{ps}[\bm k]
$$

==> tmp.tex <==
\begin{align}
    &\ddt \mathcal{N_a} - \{\phi,\mathcal{N_a}\} + \frac{\tau_a}{z_a} i k_y \squareparenthesis{2 \mathcal{N_a} + \sqrt{2} \mathcal T_{\parallel a}  - \mathcal T_{\perp a}} - i k_y\kappa_N\phi = 0 \\
    %
    &\ddt \mathcal T_{\perp a} - \{\phi,\mathcal T_{\perp a}\} + \frac{\tau_a}{z_a} i k_y \squareparenthesis{4 \mathcal T_{\perp a} + \sqrt{2} M_a^{21} -2M_a^{02}  - \mathcal{N_a}} + i k_y\kappa_T\phi = 0 \\
    %
    &\ddt \mathcal T_{\parallel a}  - \{\phi,\mathcal T_{\parallel a} \} + \frac{\tau_a}{z_a} i k_y \squareparenthesis{6 \mathcal T_{\parallel a}  + \sqrt{12}M_a^{40} + \sqrt{2} \mathcal{N_a} - M_a^{21}} - i k_y\frac{\sqrt{2}}{2}\kappa_T\phi = 0 \\
    %
    &\ddt M_a^{21} - \{\phi,M_a^{21}\} + \frac{\tau_a}{z_a} i k_y \squareparenthesis{8 M_a^{21} + \sqrt{12} M_a^{41}+ \sqrt{2} \mathcal T_{\perp a} - 2M_a^{22} - \mathcal T_{\parallel a} } = 0
    \label{eq:moment_gyboeq_explicit}
\end{align}

%% Moment equation explicit 4,2
\begin{align}
    &\Dt{N_a^{00}} + \frac{\tau_a}{z_a} i k_y \squareparenthesis{2 N_a^{00} + \sqrt{2} N_a^{20} - N_a^{01}}  
    % \nonumber\\&\qquad \qquad
    =  \squareparenthesis{\roundparenthesis{\kappa_N - 2}\kernel_0 +  ( 1- \kappa_T) \kernel_1} ik_y \phi\\
    %
    %\Dt{M_a^{10}} + \frac{\tau_a}{z_a} i k_y \squareparenthesis{4 n_a^{10} + \sqrt{6} n_a^{30} - n_a^{11}} = 0 \\
    %
    &\Dt{N_a^{20}} + \frac{\tau_a}{z_a} i k_y \squareparenthesis{6 N_a^{20} + \sqrt{12}N_a^{40} + \sqrt{2} N_a^{00} - N_a^{21}} 
    % \nonumber \\ &
    = \frac{\sqrt{2}}{2} (\kappa_T-2)  \kernel_0 ik_y  \phi\\
    %
    &\Dt{N_a^{01}} + \frac{\tau_a}{z_a} i k_y \squareparenthesis{4 N_a^{01} + \sqrt{2} N_a^{21} -2N_a^{02}  - N_a^{00}} 
    \nonumber \\ &\qquad \qquad
    =  \squareparenthesis{\roundparenthesis{1-\kappa_T}\kernel_0 +  (\kappa_N+2\kappa_T-4)\kernel_1 + (2-2\kappa_T)\kernel_2} ik_y \phi\\
    %
    %&\Dt{M_a^{30}} + \frac{\tau_a}{z_a} i k_y \squareparenthesis{8 n_a^{30} + \sqrt{20} n_a^{50} + %\sqrt{6} n_a^{10} - n_a^{31}} = 0 \\
    %
    %&\Dt{M_a^{11}} + \frac{\tau_a}{z_a} i k_y \squareparenthesis{6 n_a^{11} + \sqrt{6} n_a^{31} -2 n_a^{12} - n_a^{10}} = 0\\
    %
    &\Dt{N_a^{40}} + \frac{\tau_a}{z_a} i k_y \squareparenthesis{10 N_a^{40} \truncate{+\sqrt{30} N_a^{60}} + \sqrt{12} N_a^{20} - N_a^{41}} = 0 \\
    %
    &\Dt{N_a^{21}} + \frac{\tau_a}{z_a} i k_y \squareparenthesis{8 N_a^{21} + \sqrt{12} N_a^{41}+ \sqrt{2} N_a^{01} - 2N_a^{22} - N_a^{20}} 
    % \nonumber \\ &\qquad \qquad
    = \frac{\sqrt{2}}{2}\roundparenthesis{\kappa_T-2}\kernel_1ik_y\phi \\
    %
    &\Dt{N_a^{02}} + \frac{\tau_a}{z_a} i k_y \squareparenthesis{6 N_a^{02} + \sqrt{2} N_a^{22} \truncate{-3 N_a^{03}}  -2 N_a^{01}} = \squareparenthesis{2\kernel_1-6\kernel_2\truncate{-3\kernel_3}}ik_y\phi \\
    %
    % &\Dt{N_a^{31}} + \frac{\tau_a}{z_a} i k_y \squareparenthesis{10 n_a^{31} + \sqrt{20} n_a^{11}+ \sqrt{6} n_a^{11} - 2n_a^{32} - n_a^{30}} = 0 \\
    %
    &\Dt{N_a^{41}} + \frac{\tau_a}{z_a} i k_y \squareparenthesis{12 N_a^{41} \truncate{+ \sqrt{30} N_a^{61}}+ \sqrt{12} N_a^{21} - 2N_a^{42} - N_a^{40}} = 0 \\
    % 
    &\Dt{N_a^{22}} + \frac{\tau_a}{z_a} i k_y \squareparenthesis{10 N_a^{22} + \sqrt{12} N_a^{42}+ \sqrt{2} N_a^{02} - 3N_a^{23} - 2N_a^{21}} = -\sqrt{2}\kernel_2ik_y\phi \\
    % 
    % &\Dt{N_a^{03}} + \frac{\tau_a}{z_a} i k_y \squareparenthesis{2 n_a^{03} + \sqrt{2} n_a^{23} - 4 n_a^{04} - 3 n_a^{21}} = 0 \\
    % 
    &\Dt{N_a^{42}} + \frac{\tau_a}{z_a} i k_y \squareparenthesis{14 N_a^{42} \truncate{+ \sqrt{30} N_a^{62}}+ \sqrt{12} N_a^{22} \truncate{- 3N_a^{43}} - 2N_a^{41}} = 0 \\
     \label{eq:momenthierarchy_42}
 \end{align}

==> xx_linear_results.tex <==
\section{Linear results}
In this section we show linear results from \textsc{HeLaZ} on the growth rate of the entropy mode in a z-pinch and comparison with \textsc{Gene} for the same parameters. 
We focus on a strong density gradient drive $\kappa_N=1.8$ helped with a slight temperature gradient $\eta=25\%$ in order to avoid marginal stability region where convergence can be hard to reach in both solver.
These parameters are also chosen for comparison purpose with the work of \cite{Hallenbert2021a} whose results has been reproduced using \textsc{Gene}.
In addition to that, collisional and collisionless cases are considered, confirming the for the first time the multi-species linear Sugama collision operator in the gyromoments approach derived.
In the rest of the document we will denote the collisional frequency $\nu$ with Frei's normalization.
The equivalency for \textsc{Gene} is $\nu = 0.047 \nu_{\textsc{Gene}}$.\\
\break
The results of the linear analysis (\figref{fig:linear_analysis}) demonstrate first that \textsc{HeLaZ} retrieves \textsc{Gene} results given a large enough polynomial basis and one can see that the polynomial set required is much lower for the collisional case.
This confirms previous convergence results done on different instabilities \citep{Frei2020,Frei2021} and solidifies the idea that the gyromoment method is well suited for collisional simulation.
In addition to that, the collisional results show for the first time an agreement between \textsc{Gene} and the gyrokinetic inter-species Sugama collision operator \citep{Frei2021} used by \textsc{HeLaZ} since previous works were done using adiabatic electrons.
Finally one can notice that these results are also coherent with \textsc{GS2} results \citep{Ricci2006,Kobayashi2012} where it has been observed that collision efficiently damps the instability drive for small scale fluctuations especially in the case of gyrokinetic collision operator, i.e. including collision FLR effects.

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{figures/linear_benchmark_kn_2.0_eta_0.25.eps}
    \caption{Convergence of the linear entropy mode growth rate with respect to the result obtain with \textsc{Gene} (black) for $\kappa_N=2.0$ and $\eta=0.25$ in the collisionless case (left) and collisional case $\nu=0.05$ with Sugama model without (middle) and with FLR effects (right). The different polynomial basis resolutions used by \textsc{HeLaZ} are: $(P,J)=(4,2)$ (blue), $(P,J)=(10,5)$ (red), $(P,J)=(20,10)$ (yellow) }
    \label{fig:linear_analysis}
\end{figure}
